Charge-state dependent vibrational relaxation in a single-molecule junction

The interplay between nuclear and electronic degrees of freedom strongly influences molecular charge transport. Herein, we report on transport through a porphyrin dimer molecule, weakly coupled to graphene electrodes, that displays sequential tunneling within the Coulomb-blockade regime. The sequential transport is initiated by current-induced phonon absorption and proceeds by rapid sequential transport via a non-equilibrium vibrational distribution. We demonstrate this is possible only when the vibrational dissipation is slow relative to sequential tunneling rates, and obtain a lower bound for the vibrational relaxation time of 8 ns, a value that is dependent on the molecular charge state.

==> def.tex <==
\newcommand{\R}{{\cal{R}}}
\def\nat#1#2#3{Nature {\bf #1}, #2 (#3)}
\def\np#1#2#3{Nat. Phys. {\bf #1}, #2 (#3)}
\def\sc#1#2#3{Science {\bf #1}, #2 (#3)}
\def\prv#1#2#3{Phys. Rev. {\bf #1}, #2 (#3)}
\def\rmp#1#2#3{Rev. Mod. Phys. {\bf #1}, #2 (#3)}
\def\prl#1#2#3{Phys. Rev. Lett. {\bf #1}, #2 (#3)}
\def\pra#1#2#3{Phys. Rev. A {\bf #1}, #2 (#3)}
\def\prb#1#2#3{Phys. Rev. B {\bf #1}, #2 (#3)}
\def\prd#1#2#3{Phys. Rev. D {\bf #1}, #2 (#3)}
\def\pre#1#2#3{Phys. Rev. E {\bf #1}, #2 (#3)}
\def\epl#1#2#3{Europhys. Lett. {\bf #1}, #2 (#3)}
\def\epjb#1#2#3{Eur. Phys. J. B {\bf #1}, #2 (#3)}
\def\epjd#1#2#3{Eur. Phys. J. D {\bf #1}, #2 (#3)}
\def\njp#1#2#3{New J. Phys. {\bf #1}, #2 (#3)}
\def\jstat#1#2#3{J. Stat. Mech. {\bf #1}, #2 (#3)}
\def\jpamt#1#2#3{J. Phys. A: Math. Theor. {\bf #1}, #2 (#3)}
\def\jpamg#1#2#3{J. Phys. A: Math. Gen. {\bf #1}, #2 (#3)}
\def\jpb#1#2#3{J. Phys. B: At. Mol. Opt. Phys. {\bf #1}, #2 (#3)}
\def\jpcm#1#2#3{J. Phys.: Cond. Matt. {\bf #1}, #2 (#3)}
\def\jpcs#1#2#3{J. Phys.: Conf. Ser. {\bf #1}, #2 (#3)}
\def\pr#1#2#3{Phys. Rep. {\bf #1}, #2 (#3)}
\def\pl#1#2#3{Phys. Lett. {\bf #1}, #2 (#3)}
\def\pla#1#2#3{Phys. Lett. A {\bf #1}, #2 (#3)}
\def\plb#1#2#3{Phys. Lett. B {\bf #1}, #2 (#3)}
\def\physa#1#2#3{Physica A {\bf #1}, #2 (#3)}
\def\jsp#1#2#3{J. Stat. Phys. {\bf #1}, #2 (#3)}
\def\jltp#1#2#3{J. Low Tem. Phys. {\bf #1}, #2 (#3)}
\def\lpl#1#2#3{Laser Phys. Lett. {\bf #1}, #2 (#3)}
\def\lp#1#2#3{Laser Phys. {\bf #1}, #2 (#3)}
\def\apl#1#2#3{Appl. Phys. Lett. {\bf #1}, #2 (#3)}
\def\ajp#1#2#3{Am. J. Phys. {\bf #1}, #2 (#3)}
\def\epj#1#2#3{Eur. Phys. J. {\bf #1}, #2 (#3)}
\def\jmp#1#2#3{J. Math. Phys. {\bf #1}, #2 (#3)}
\def\lanl{{\it LANL archives}}
\def\etc{etc.}
\def\half{\frac{1}{2}}
\def\ie{i.e.}
\def\H{{\cal H}}
\def\Hp{H_1}
\def\eff{\mathrm{eff}}
\def\q{\qquad}
\def\i{\indent}
\def\noi{\noindent}
\def\bc{\begin{center}}
\def\ec{\end{center}}
\topmargin=-1.5cm
\newcommand{\bea}{\begin{equation}}
\newcommand{\eea}{\end{equation}\noi}
\newcommand{\ber}{\begin{eqnarray}}
\newcommand{\eer}{\end{eqnarray}\noi}
\textheight=23.0cm

